POSSCORE: A Simple Yet Effective Evaluation of Conversational Search with Part of Speech Labelling

Conversational search systems, such as Google Assistant and Microsoft Cortana, provide a new search paradigm where users are allowed, via natural language dialogues, to communicate with search systems. Evaluating such systems is very challenging since search results are presented in the format of natural language sentences. Given the unlimited number of possible responses, collecting relevance assessments for all the possible responses is infeasible. In this paper, we propose POSSCORE, a simple yet effective automatic evaluation method for conversational search. The proposed embedding-based metric takes the influence of part of speech (POS) of the terms in the response into account. To the best knowledge, our work is the first to systematically demonstrate the importance of incorporating syntactic information, such as POS labels, for conversational search evaluation. Experimental results demonstrate that our metrics can correlate with human preference, achieving significant improvements over state-of-the-art baseline metrics.

==> content/9_discussion_archive_.tex <==
% length bias
% learning methods
% Embedding selection
%normalize
\begin{comment}
\begin{table*}[]
\begin{tabular}{l|c|c|c|c}
\hline
Reference & \multicolumn{4}{l}{i like sports , football , hockey , soccer i also find swimming interesting as well .} \\
Good candidate & \multicolumn{4}{l}{i like hockey and soccer . what teams do you support ?} \\
Bad candidate & \multicolumn{4}{l}{i have never swam competitively , but i did nt have it . i do like it though .} \\ \hline
POS tag set & \multicolumn{4}{c}{PROPN + NOUN + ADV + PRON} \\ \hline
 & POS number & $w$ & S(POS) & POSSCORE \\ \hline
Reference & 10 & - & - & - \\
Good candidate & 6 & 0.513 & 0.848 & 1.274 \\
Bad candidate & 9 & 0.895 & 0.681 & 1.391 \\ \hline
\end{tabular}
\caption{A failure example of POSSCORE. POS number means the number of POS words in the sentence. $w$ is the weight value of POS similarity part. S(POS) denotes the similarity score of POS word sequence. Although the similarity of POS part in the good candidate is higher than that in the bad candidate, the biased weight $w$ increase the final POSSCORE of bad one. }
\label{tab:example_posscore}
\end{table*}
\end{comment}





 Our proposed evaluation metrics use a simple approach to incorporate POS distribution information in conversational search evaluation. Our results show that our new POSSCORE metric consistently achieves better performance than the widely-used baselines, for different collections. However, there are still some discussion points of our experiment:
 \begin{itemize}
%     \item The weight function $w$ may have a bias to the candidates which contain more number of POS tags. If one candidate has more POS words, the weight function may tend to give higher weight scores. Since we simply use the quotient of the number of POS words between references and candidates to capture the connection of POS distribution, the weight function could be sensitive to the number of POS words. Table ~\ref{tab:example_posscore} presents a failure case due to the weight bias. We can see that since the POS number of bad candidate is more than that of good one, $w$ of bad candidate becomes higher than that of good one. Although the POS similarity score of the bad candidate is smaller than the score of good one, the weight $w$, to some extent, increases the importance of POS part in bad candidate. Therefore, the final POSSCORE judgement is opposite to the human preference in this case. To reduce this bias, a simple solution is to normalize the number of POS words when calculating the weight function. We leave the design of normalization approaches in the future work.
     
%     \item We have not yet considered BERTScore (a embedding-based metric) and BERT-RUBER (a learning-based metric), which are also the state-of-the-art metrics in open-domain dialogue evaluation, because the main goal of our experiment is to identify and measure the influence of POS tags in the evaluation process, and compare the difference between with and without POS words. It is difficult to design a simple method to incorporate the POS information into these other metrics. For example, BERTScore capture the corpus-level idf of each word. If we only use POS words to perform BERTScore, this may change the word distribution of the whole corpus and have an influence on the idf parameter. This makes it difficult to interpret the effect of POS tags. Therefore, we select popular but simple structure metrics as our baselines.

     \item The length bias of metrics. Since POSSCORE counting the number of POS and Non-POS words and tags, we concern about the influence of response length on the performance of POSSCORE. To examine the effect of length bias, we build a new datasets, where we duplicate the bad responses once and concatenate the duplicated response to the original bad responses. Thus, all the bad responses is as twice long as original bad responses. Then, in this new bad long-response datasets, we use BLEU2, BLEU4, METEOR, EA and POSSCORE to examine the influence of response length. Table ~\ref{tab:length_bias} presents the predictive power results of different metrics. It can be observed that POSSCORE are not significantly affected by the length variation of bad responses. All the results of POSSCORE are better than other baseline metrics. Therefore, we can see the proposed POSSCORE can free from the length bias effects.
     
     \item The choice of word embedding may also affect the performance of POSSCORE. In this paper, we only present the results of Fasttext embedding. Since the POS and Non-POS similarity scores are computed on the word embedding, embedding methods may also play a vital role in POSSCORE. We also leave this part in the future work. 
     
     \item POSSCORE only concentrates on the difference between references and candidates, and evaluates the candidate response against the gold standard references. In conversational search, conversation context may also contain useful explicit and implicit information for evaluation. Using POS words to extract key information from context may also be helpful for future evaluation and metric design.
 \end{itemize}
 
\begin{table}[t] \small
\begin{tabular}{c|ccc}
\hline
         & TC             & PC            & MSDialog       \\ \hline
BLEU2    & 0.718          & 0.652         & 0.535          \\
BLEU4    & 0.715          & 0.698         & 0.541          \\
METEOR   & 0.653          & 0.616         & 0.508          \\
EA       & 0.642          & 0.662         & 0.556          \\ \hline
POSSCORE & \textbf{0.756} & \textbf{0.71} & \textbf{0.587} \\ \hline
\end{tabular}
\caption{The predictive power results of bad long-response test. Each of bad candidate responses is duplicated once. Thus, all the bad responses have double length of the original bad responses. }
\label{tab:length_bias}
\vspace{-0.2in}
\end{table}



